OpenReq Issue Link Map: A Tool to Visualize Issue Links in Jira

Managing software projects gets more and more complicated with an increasing project and product size. To cope with this complexity, many organizations use issue tracking systems, where tasks, bugs, and requirements are stored as issues. Unfortunately, managing software projects might remain chaotic even when using issue trackers. Particularly for long lasting projects with a large number of issues and links between them, it is often hard to maintain an overview of the dependencies, especially when dozens of new issues get reported every day. We present a Jira plug-in that supports developers, project managers, and product owners in managing and overviewing issues and their dependencies. Our tool visualizes the issue links, helps to find missing or unknown links between issues, and detects inconsistencies.

==> annex.tex <==
\section*{Annex}
\subsection{Goal of the demo}
We want to get feedback on the features and the visualization from experts (academia and companies) to improve the tool. Additionally, we want to hear from other users how they are dealing with similar problems.

\subsection{How the tool will be presented}
We will present \emph{OpenReq Issue Link Map} in an interactive and live tool demonstration and with a poster explaining the problem and showcasing the features of the tool. The audience can search for different issues in Qt's Jira, look and explore the issue link maps and try the link detection and the consistency checker. A easy to understand toy project that shows the different features could be created for the conference.

\textbf{Interactive Demonstration.}
The tool can be reached under the following url: \url{https://api.openreq.eu/openreq-issue-link-map/}.
At the conference, interested persons are free to interact with the tool as they wish. Some features are still in developement and may not be bug-free until the conference.
%At the point of the conference the tool might be universial applicable to every Jira and a test jira can be hosted locally

The European Horizon 2020 project OpenReq and its goals will be introduced as well.
We further explain how and why we are developing the tool and in which industry scenarios it is currently tested and useful. Additionally, we will describe how the tool can be used in other circumstances apart from Qt's environment.

\textbf{Poster.}
A poster (see~\ref{fig:Poster} that introduces the problem and explains the features will be provided, so that interested persons can learn about the tool and what it does prior to trying it out. This way the audience has a way to familiarize with the tool and a guide to refer to while they are using the tool. As the UI is not described in full detail in the tool paper itself, the focus of the poster will be on the different UI elements and their functions so that the user can achieve a better understanding of the OpenReq Issue Link Map.

%check with Mikko H
% \textbf{Video.}
% We will also show a video which showcases the features of the \emph{OpenReq Issue Link Map}.

\subsection{Further documentation}
Every component of the European Horizon 2020 project OpenReq is open source, and so are all microservices of \emph{OpenReq Issue Link Map}\footnote{\url{https://github.com/OpenReqEU}}.
Despite the code being publicly available, we also document all API endpoints of our components\footnote{\url{https://api.openreq.eu}}.
In our demonstration, we will direct the audience to both points since all parts of the OpenReq project can be used stand-alone in a requirements engineering context.

\clearpage
\begin{figure*}[tb]\label{fig:Poster}
    \centering
    \includegraphics[width=\textwidth]{pics/REToolDemoPoster_port.pdf}
    \caption{Poster for Tool Demo}
\end{figure*}
